Imaging the inner astronomical unit of Herbig Be star HD 190073

Inner regions of protoplanetary disks host many complex physical processes such as star-disk interactions, magnetic fields, planet formation, and the migration of new planets. To directly study this region requires milli-arcsecond angular resolution, beyond the diffraction limit of the world's largest optical telescopes and even too small for the mm-wave interferometer ALMA. However, we can use infrared interferometers to image the inner astronomical unit. Here, we present new results from the CHARA and VLTI arrays for the young and luminous Herbig Be star HD 190073. We detect a sub-AU cavity surrounded by a ring-like structure that we interpret as the dust destruction front. We model the shape with 6 radial profiles, 3 symmetric and 3 asymmetric, and present a model-free image reconstruction. All the models are consistent with a near face-on disk with inclination $\lesssim 20^\circ$, and we measure an average ring radius of 1.4 $\pm 0.2$ mas (1.14 AU). Around $48\%$ of the total flux comes from the disk with ~$15\%$ of that emission appearing to emerge from inside the inner rim. The cause of emission is still unclear, perhaps due to different dust grain compositions or gas emission. The skewed models and the imaging point to an off-center star, possibly due to binarity. Our image shows a sub-AU structure, which seems to move between the two epochs inconsistently with Keplerian motion and we discuss possible explanations for this apparent change.

==> v1295.tex <==
Images were reconstructed using conventional regularized maximum likelihood and the open source OITOOLS.jl
package \citep{Martinez2021} \footnote{\url{https://github.com/fabienbaron/OITOOLS.jl}}.
Only powerspectra and closure phases were used for the reconstructions.

In line with previous mixed modeling and imaging works (e.g. SPARCO in \citet{Kluska2014}), the
star was modeled as a point source in the center of the field of view,
of spectrum proportional to $\lambda^4$, while the environment was
assumed to follow a $\lambda^\alpha$ dependency, with $\alpha$ free to
vary. In addition we modeled potential extended or background emission
as a zero visibility component, also following $\lambda^4$. Thus there
were three free parameters in addition to image pixels: $\alpha$ and
the flux ratios disk/star and extended emission/star.

Minimization was ensured by the gradient-based
VMLM-B \citep{Thiebaut2002} algorithm from OptimPack, enforcing
positivity of the disk intensity. Three other priors were employed in
addition to positivity: compactness to regularize large scale
emission, total variation to handle small scale pixel correlations
(see e.g. \citep{Thiebaut2017} for the mathematical expression of
these), as well as a novel azimuthal regularization to "circularize"
YSO disks at medium scales. Given four hyperparameters (the centroid,
inclination and position angle of the disk), this regularizer simply
computes the location of concentric elliptical rings, and then sums
the azimuthal pixel variances along them. Minimizing the regularizer
enforces relative smoothness along the rings, but unlike total
variation . Since the expression can be written as a squared $\ell_2$
norm of a linear operator on the image, it lends itself well to the
gradient-based approach. Hyperpriors for the four hyperparameters were
uniform and an initial hyperparameter range was roughly determined
from the data by directly minimizing the variance of the de-rotated
powerspectra. The Nelder-Mead simplex was used to optimize the four
hyperparameters, new reconstructions were run with different sets of
hyperparameters until a global minimum was found. Values for the other
regularization hyperparameters were chosen based on quick simulations
(copying the uv coverage and signal-to-noise of the actual data and
reconstructing disks), within the expected range \citep{Renard2011}.
The final reduced $\chi^2$ for the images is $\chi^2_\text{v2} \simeq
1.05$ and $\chi^2_\text{t3phi}\simeq 0.85$ for epoch A and $\chi^2_\text{v2} \simeq
0.95$ and $\chi^2_\text{t3phi}\simeq 1.1$ for epoch B. 


@ARTICLE{Kluska2014,
       author = {{Kluska}, J. and {Malbet}, F. and {Berger}, J. -P. and {Baron}, F. and {Lazareff}, B. and {Le Bouquin}, J. -B. and {Monnier}, J.~D. and {Soulez}, F. and {Thi{\'e}baut}, E.},
        title = "{SPARCO : a semi-parametric approach for image reconstruction of chromatic objects. Application to young stellar objects}",
      journal = {\aap},
     keywords = {methods: numerical, techniques: high angular resolution, techniques: interferometric, protoplanetary disks, stars: variables: T Tauri, Herbig Ae/Be, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = apr,
       volume = {564},
          eid = {A80},
        pages = {A80},
          doi = {10.1051/0004-6361/201322926},
archivePrefix = {arXiv},
       eprint = {1403.3343},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...564A..80K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Thiebaut2002,
       author = {{Thi{\'e}baut}, {\'E}ric},
        title = "{Optimization issues in blind deconvolution algorithms}",
    booktitle = {Astronomical Data Analysis II},
         year = 2002,
       editor = {{Starck}, Jean-Luc and {Murtagh}, Fionn D.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {4847},
        month = dec,
        pages = {174-183},
          doi = {10.1117/12.461151},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002SPIE.4847..174T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Renard2011,
       author = {{Renard}, S. and {Thi{\'e}baut}, E. and {Malbet}, F.},
        title = "{Image reconstruction in optical interferometry: benchmarking the regularization}",
      journal = {\aap},
     keywords = {instrumentation: interferometers, techniques: interferometric, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = sep,
       volume = {533},
          eid = {A64},
        pages = {A64},
          doi = {10.1051/0004-6361/201016263},
archivePrefix = {arXiv},
       eprint = {1106.4508},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...533A..64R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Thiebaut2017,
       author = {{Thi{\'e}baut}, {\'E}ric and {Young}, John},
        title = "{Principles of image reconstruction in optical interferometry: tutorial}",
      journal = {Journal of the Optical Society of America A},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = jun,
       volume = {34},
       number = {6},
        pages = {904},
          doi = {10.1364/JOSAA.34.000904},
archivePrefix = {arXiv},
       eprint = {1708.08390},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017JOSAA..34..904T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

